Smoothed Analysis of Social Choice, Revisited

A canonical problem in social choice is how to aggregate ranked votes: given $n$ voters' rankings over $m$ candidates, what voting rule $f$ should we use to aggregate these votes into a single winner? One standard method for comparing voting rules is by their satisfaction of axioms - properties that we want a "reasonable" rule to satisfy. Unfortunately, this approach leads to several impossibilities: no voting rule can simultaneously satisfy all the properties we want, at least in the worst case over all possible inputs. Motivated by this, we consider a relaxation of these worst case requirements. We do so using a "smoothed" model of social choice, where votes are perturbed with small amounts of noise. If, no matter which input profile we start with, the probability (post-noise) of an axiom being satisfied is large, we will consider the axiom as good as satisfied - called "smoothed-satisfied" - even if it may be violated in the worst case. Our model is a mild restriction of Lirong Xia's, and corresponds closely to that in Spielman and Teng's original work on smoothed analysis. Much work has been done so far in several papers by Xia on axiom satisfaction under such noise. In our paper, we aim to give a more cohesive overview on when smoothed analysis of social choice is useful. Within our model, we give simple sufficient conditions for smoothed-satisfaction or smoothed-violation of several previously-unstudied axioms and paradoxes, plus many of those studied by Xia. We then observe that, in a practically important subclass of noise models, although convergence eventually occurs, known rates may require an extremely large number of voters. Motivated by this, we prove bounds specifically within a canonical noise model from this subclass - the Mallows model. Here, we present a more nuanced picture on exactly when smoothed analysis can help.

==> 4results2.tex <==





\section{Beyond dependence on the minimum probability}\label{sec:beyond-minprob}

The convergence rates to smoothed-satisfaction in \Cref{sec:positive-results} --- and those in the related work \cite{xia2020smoothed} --- depend on $1/\sqrt{n\minprob^3}$. This means that when $\minprob$ is very small, extremely large $n$ is required to get reasonably low probability of an axiom violation: for example, per the relative $n$ and $\minprob$ dependency in \Cref{prop:resolvability}, if we decrease $\minprob$ by a factor of 10, we need to increase $n$ by a factor of 1000 in order to recover the same probability bound.\footnote{One may wonder if different techniques could potentially improve this dependence. Although we do not have a tight cubic lower bound and the exact bound should depend on the exact voting rule/axiom, we can at least get a linear one. Indeed, consider the noise distribution that switches to any ranking other than the starting one with probability $\varepsilon$, but stays on the starting one with probability $1 - (m! - 1)\varepsilon$. The minimum probability here is $\varepsilon$, but we need $n \in \omega(\varepsilon / m!)$ to ensure that the profile changes at all with high probability, a necessary condition to smoothed-satisfy any axiom that fails on even a single profile.}
 %
 %For example in the mallows model, to get probability of success $0.95$ with noise level of $0.1$, we need $n = XXX$ voters in the election.
%
%Unfortunately, noise models in which $\minprob$ is very small represent an extremely practically important subclass of noise models: they encompass any noise model in which small perturbations are unlikely to \textit{completely reverse} someone's ranking. In reality, this is almost a precondition for a smoothed model of social choice to be realistic: the small real-world shocks that may perturb people's preferences are unlikely to qualitatively change their opinions to the extent that their rankings are reversed.

Motivated by the importance of noise models in which $\minprob$ is small (per the introduction), we now pursue convergence bounds parameterized by values other than $\minprob$. Although many of our ideas here would naturally extend to broader classes of noise models, for concreteness, we prove bounds specifically within the \textit{Mallows model}, a well-established and well-characterized noise model over rankings. The noise added by this model makes rankings with more swaps less likely, as desired.
\begin{definition}[Mallows noise model \cite{mallows1957non}]\label{def:mallows}
Let $d : \rankings \times \rankings \to \mathbb{N}$ be the Kendall-Tau distance. Then, the Mallows model $\noisemodel^{Mallows}_\phi$ is defined as follows, where $Z = \sum_{\ranking' \in \rankings} \phi^{d(\ranking',\ranking)}$, a normalizing term.
\[\Pr\left[\noisemodel^{Mallows}_{\phi}(\ranking) = \ranking'\right] = \frac{1}{Z} \phi^{d(\ranking,\ranking')}.\]
\end{definition}

Within this model, we will study at what rates different voting rules smoothed satisfy \textsc{Resolvability} and $\rho(n)$\textsc{-Group-Stability}\emdash the two axioms we know from \Cref{sec:positive-results} to be smoothed-satisfied by most rules we study. Of course, because the Mallows model satisfies \Cref{ass:extremal,ass:continuity,ass:positivity,ass:monotonicity}, we immediately inherit these smoothed-satisfaction rates. However, we can now concretely see that these bounds are not very practically useful because $\minprob(\noisemodel^{Mallows}_\phi)$ is exponentially small in $m$: noting that the maximum Kendall-Tau distance between rankings is $\binom{m}{2}$, $\minprob(\noisemodel^{Mallows}_\phi) \in \phi^{\Omega(m^2)}$. %This means that $n$ needs to grow extremely quickly as $m$ grows to retain good $\minprob$-parameterized bounds. For example, suppose $\phi$ is fixed at $1/2$ and we increase $m$ from $2$ to $3$; we then need to increase $n$ by a factor of $2^{\binom{3}{2}*3/2 - \binom{2}{2}*3/2} = 8$ in order to maintain the same probability of post-noise satisfaction. 

In the next sections, we will prove various bounds on convergence rates as functions of $m$ and $\phi$. However, in \Cref{tab:classification4}, we summarize our bounds in a slightly different way. Namely, how large must $n$ be to ensure satisfaction with high probability? We distinguish here between rules/axioms in which $n$ needs only be polynomial in $m$ and $1/\phi$ (which we view as a reasonable requirement) versus those where $n$ is necessarily exponential. We focus specifically on the axiom \textsc{Resolvability}. What these bounds show is a clear separation between voting rules: \textsc{Plurality} and \textsc{Borda} have reasonable requirements, while \textsc{Minimax} and \textsc{Veto} do not. 

The proofs of these results are located in \Cref{sec:proofs}; there, we discuss why essentially the same results should hold for noise models beyond the Mallows model which make large opinion change unlikely, or even occur with probability zero.

\begin{table}[h!]
    \centering
    \begin{tabular}{r||cc}
        & \multicolumn{2}{c}{\textbf{Axioms}}\\
           \textbf{Voting Rules}&  \textsc{Resolvability}  &  \textsc{$\sqrt{n}$-Group Stability$^*$}\\
         \hline \hline \\[-0.9em]
         \textsc{Plurality} & $\omega(m^5/\phi)$ suff. &  \\[0.25em]
        \textsc{Borda} &  $\omega\left(m^6 / \phi\right)$ suff.  &  \\[0.25em]
                \hline \\[-0.9em]
        \textsc{Veto} & $\Omega(1/\phi^{m - 2})$ necc.&\\
        \textsc{Minimax} & $\Omega\left(1/(m\phi^{m/2}\right)$ necc. & 
    \end{tabular}
    \caption{}
    \label{tab:classification4}
\end{table}
% \textcolor{red}{did some simplifications to get the gist - we should check.}

% To help make clear the practical separation of voting rules implied by these $\phi$ dependencies, consider the following example. Suppose we increase the number of alternatives from $m$ to $m' > m$; we will study, for each voting rule, by what factor we need to increase the number of voters $n$ to maintain the same convergence rate. For \textsc{Plurality} and \textsc{Borda}, we must increase $n$ by a factor of $(m'/m)^5$ and $(m'/m)^6$,  respectively; in contrast, for \textsc{Veto} and \textsc{Minimax}, we need to increase the $n$ by a factor of $1/\phi^{m' - m}$ and $m/m' \cdot 1/\phi^{(m'-m)/2}$, respectively. To put this in perspective, Suppose $\phi = 1/10$ and we increase the number of alternatives from $m = 2$ to $m = 5$. The values for pl


% \textbf{\textcolor{red}{Extra text that might be useful: }} \textcolor{red}{Interestingly, we show that $\minprob$-dependent bounds hide a lot of diversity among voting rules in terms of the rates at which they converge to smoothed-satisfaction of \textsc{Resolvability} and $\rho(n)$\textsc{-Group-Stability}. Some only require a number of voters polynomial in the noise and number of candidates, while for others, this dependence is exponential. As summarized in \Cref{tab:classification4}, we find that for many voting rules, convergence rates \textit{must remain at least exponential in $m$}. This occurs for voting rules whose winners are not that sensitive to low-Kendall-Tau-distance changes in rankings: take the example of \textsc{Veto}, where swaps in the first $m-1$ positions do not change the scores of any alternative.
% In contrast, voting rules whose winners are more sensitive to such local perturbations ....
% %
% What this reveals is a more nuanced picture of when smoothed analysis is useful: for some rules and axioms, smoothed analysis is not actually that useful \textit{unless we permit small amounts of noise to translate to qualitative shifts in individuals' opinions with somewhat high probability.}}




\subsection{Technical Analysis} \label{sec:proofs}
For these proofs, we will need several known properties of the Mallows model. First, from \cite{awasthi2014learning}, we have%
%an alternative equivalent way of sampling that allows us to reason about certain properties of the final rankings. Namely, to sample a ranking from a Mallows model centered at $\sigma$, we can iteratively construct the ranking by first choosing the top candidate to be the $j$'th candidate $\sigma(j)$ with probability proportional to $\phi^j$, so with probability $\frac{\phi^j}{\sum_{j' = 1}^m \phi^{j'}}$. We can then recurse on the rest of the ranking, drawing it from a Mallows distribution centered at $\sigma$ with chosen candidate $\sigma(j)$ removed. Note that this implies
that each candidate $\sigma(j)$ ends up first with probability proportional to $\phi^j$, i.e., $\frac{\phi^j}{\sum_{j' = 1}^m \phi^{j'}}$. Symmetrically, a candidate ranked $j$ will end up last with probability proportional to $\phi^{m - j}$. %
%Further, the top two candidates $\sigma(1)$ and $\sigma(2)$ will remain in their positions with probability $\frac{\phi}{\sum_{j' = 1}^m \phi^{j'}} \cdot \frac{\phi}{\sum_{j' = 1}^m \phi^{j'}}$. 
Additionally, from \cite{mallows1957non}, if two candidates are a distance $k$ apart in the ranking, i.e., $\sigma(i)$ and $\sigma(j)$ with $i - j = k$, the probability they retain their relative orders in the sampled ranking is increasing in $k$ (and always at least $1/2$). This was refined by \cite{mallowsprobbound} to an exact value
    \[q(k) := \frac{1}{1-\phi^{k+1}}\left(1 - \frac{(1-\phi)k\phi^k}{1 - \phi^k}\right).\]
We will in general parameterize our bounds by the probability a swap \emph{does} occur at a distance of $k$, which we define to be $\bar{q}(k) := 1 - q(k)$.
To gain more intuition for these bounds, it will be useful to derive some lower bounds on $q(k)$ (corresponding to upper bounds on $\bar{q}(k)$. Depending on the exact relationship between $m$ and $\phi$, different ones will be more useful than others.
First, we have that
\[
    q(k) = \frac{1}{1-\phi^{k+1}}\left(1 - \frac{(1-\phi)k\phi^k}{1 - \phi^k}\right) \ge 1 - \frac{(1-\phi)k\phi^k}{1 - \phi^k} \ge 1 - k\phi^k.
\]  
Second,
\begin{align*}
    q(k) &= \frac{1}{1-\phi^{k+1}}\left(1 - \frac{(1-\phi)k\phi^k}{1 - \phi^k}\right)\\
    &\ge 1 - \frac{(1-\phi)k\phi^k}{1 - \phi^k}\\
    &= 1 - \frac{k\phi^k}{\sum_{j = 0}^{k - 1}\phi^j}\\
    &= 1 - \frac{k}{\sum_{j = 0}^{k - 1}\phi^{j-k}}\\
    &= 1 - \frac{1}{\frac{1}{k}\sum_{j = 1}^{k} \frac{1}{\phi^j}}\\
    &\ge 1 - \frac{1}{\left(\prod_{j = 1}^{k} \frac{1}{\phi^j}\right)^{1/k}}\\
    &= 1 - \phi^{\frac{k(k + 1)}{2} \cdot \frac{1}{k}} = 1 - \phi^{\frac{k + 1}{2}} \ge 1 - \phi^{k/2}\\
    &
\end{align*}
where the second inequality holds due to the AM-GM inequality.
And third,
\[
    q(k) \ge q(1) = \frac{1}{1 - \phi^2}\left(1 - \frac{(1 - \phi)\phi}{1 - \phi}\right) = \frac{1 - \phi}{1 - \phi^2} = \frac{1}{1 + \phi} = 1 - \frac{\phi}{1 + \phi}
\]

These give us three upper bounds on the probability of a swap $\bar{q}(k)$, $k\phi^k, \phi^{k/2}$, and $\frac{\phi}{1 + \phi}$.

\textbf{Plurality.}
\begin{proposition}
    \textsc{Plurality} smoothed-satisfies \textsc{resolvability} at a rate of
    \[O\left(m\exp\left(-\frac{n}{6m}\right) + \frac{m^\frac{5}{2}}{\sqrt{n} \phi^{\frac{1}{2}}}  \right).\]
\end{proposition}
\begin{proof}
Fix a starting profile $\profile$.
For a candidate $c$, let $X^c_i$ be the indicator that voter $i$ ranks $c$ first and let $p^c_i = \Pr[X^c_i = 1]$. Note that in a Mallows model, the probability a candidate ranked in position $j$ ends up in the first position is proportional to $\phi^j$~\cite{awasthi2014learning}. Therefore, each $p_i$ is upperbounded by $\frac{\phi}{\sum_{j = 1}^m \phi^j} \le \frac{\phi}{\phi + \phi^2} = \frac{1}{1 + \phi}$ (since we are assuming $m \ge 2$).   Let $S^c = \sum_i X^c_i$ be the random variable for the plurality score of $c$.

We will partition the candidates into two sets, this with $L = \mathbb{E}[S^a] < \frac{n}{2m}$ and those with $H = \mathbb{E}[S^a] \ge \frac{n}{2m}$. We will first show that, except with an exponentially small probability, the winner will be from $H$. Then, we will show that the probability any two candidates in $H$ have the same plurality score is small. Union bounding over these two events will upper boudn the probaility of an unresolvable plurality tie.


Fix a candidate $a \in L$. Note that a necessary condition for $a$ to be a plurality winner is for their score to be at least $n/m$. Standard Chernoff bounds say this should happen with probability at most $\exp(-\frac{n}{6m})$. Hence, the probability any candidate in $L$ wins is at most $|L| \exp(-\frac{n}{6m})$.

Next, fix two candidates $a, b \in H$. Let $Y_i = X^a_i - X^b_i$. We can upperbound $\Pr[S^a = S^b]$ by $\Pr[\sum_i Y_i = 0]$. By Berry-Esseen, since a the Normal distribution places $0$ mass on any point,w e can lower bound this by the convergence rate which is $O\left(\frac{1}{\sqrt{\sum_i \sigma_i^2}} \max_i \frac{\rho_i}{\sigma_i^2} \right)$ where $\sigma_i^2 = \mathbb{E}[(Y_i - \mathbb{E}[Y_i])^2]$ is the variance of $Y_i$ and $\rho_i = \mathbb{E}[|Y_i - \mathbb{E}[Y_i]|^3$. Note that since each $Y_i \in [-1, 1]$, $|Y_i - \mathbb{E}{Y_i}| \le 2$, so $\max_i \frac{\rho_i}{\sigma_i^2} \le 2$. 
Expanding out $\Var[Y_i]$, we get 
\[\Var[Y_i] = \mathbb{E}[Y_i^2] - \mathbb{E}[Y_i]^2 = E[(X_i^{a})^2] + E[(X_i^{b})^2]- 2E[X_i^{a}X_i^{b}] - E[X_i^{a} - X_i^{b}]^2 = p_i^a + p_i^b - (p_i^a - p_i^b)^2,\]
using that $2E[X_i^{a}X_i^{b}] = 0$, because only one of these indicators can be 1 for a given agent $i$. We then have that, \[(p_i^a - p_i^b)^2 \le \max(p_i^a, p_i^b)^2 \le \max(p_i^a, p_i^b) (p_i^a + p_i^b) \le \frac{1}{1 + \phi}(p_i^a + p_i^b),\]
Using this, we have \[
\Var[Y_i] \ge p^a_i + p^b_i -  \frac{1}{1 + \phi}(p_i^a + p_i^b) = \frac{\phi}{1 + \phi}(p_i^a + p_i^b).\] Therefore, $\sum_i \Var[Y_i] \ge \frac{\phi}{1 + \phi}(\mathbb{E}[S^a] + \mathbb{E}[S^b]) \ge \frac{\phi}{1 + \phi} \cdot \frac{n}{m} \ge \frac{\phi}{2} \cdot \frac{n}{m}$. So Berry-Esseen implies that this occurs with probability at most
\[
    O\left(\frac{m^\frac{1}{2}}{\sqrt{n} \phi^{\frac{1}{2}}}  \right).
\]
Union bounding over the at most $|H|^2$ pairs of candidates in $H$, the probability such a tie occurs is at most $O\left(|H|^2 \frac{m^\frac{1}{2}}{\sqrt{n} \phi^{\frac{1}{2}}} \right)$. Using that both $|L| \le m$ and $|H| \le m$, we have that the overall probability of a tie is at most
\[
    O\left(m\exp\left(-\frac{n}{6m}\right) + \frac{m^\frac{5}{2}}{\sqrt{n} \phi^{\frac{1}{2}}}  \right). \qedhere
\]
\end{proof}
This means $n \in \omega\left(\frac{m^5}{\phi}\right)$ is sufficient to ensure satisfaction with high probability. Note that the main requirement on the noise model here is that no position is ranked first with probability near $1$. Any noise model where this is bounded away would lead to a similar bound.

\textbf{Borda.}
\begin{proposition}
    \textsc{Borda} smoothed-satisfies \textsc{Resolvability} at a rate of
    \[
        O\left(\frac{m^3}{\sqrt{n\phi}}\right)
    \]
\end{proposition}
\begin{proof}
    Fix a starting profile $\profile$. Fix two candidates $a$ and $b$. We will upper bound the probability that $a$ and $b$ have the same Borda score and then union bound over all pairs of candidates. For a candidate $c$, let $X^c_i$ be a random variable taking on (integer) values in $[0, m - 1]$ representing the Borda score given to candidate $c$ by voter $i$ after sampling their ranking. Let $Y_i = X^a_i - X^b_i$ be the difference in Borda score given to $a$ and $b$ by voter $i$. We would like to upper bound $\Pr[\sum_i Y_i = 0]$. Similar to the proof for \textsc{Plurality}, we use Berry-Esseen. As the normal distribution places zero mass on the value zero, we simply upper bound it by the convergence rate, $O\left(\frac{1}{\sqrt{\sum_i \sigma_i^2}} \max_i \frac{\rho_i}{\sigma_i^2} \right)$. Note that $Y_i \in [-(m - 1), (m - 1)]$, so $|Y_i - \mathbb{E}[Y_i]| \le 2m$, implying the same bound on $\max_i \frac{\rho_i}{\sigma_i^2}$. To lower bound each $\sigma_i^2$, we consider the distribution of $Y_i$. In particular, we will upper bound the probability of any specific (integer) value by $\frac{1}{1 + \phi}$. That is, for all values $\ell$,
    \begin{equation}\label{eq:mode-bound}
        \Pr[Y_i = \ell] \le \frac{1}{1 + \phi}
    \end{equation}
    Once we have shown Inequality~\eqref{eq:mode-bound} holds, note that at most one value $\ell$ can be within $1/2$ of $\E[Y_i]$, so this will imply that with probability at least $1 - \frac{1}{1 + \phi} = \frac{\phi}{1 + \phi} \ge \frac{\phi}{2}$, $|Y_i - \mathbb{E}[Y_i]| \ge 1/2$. This allows us to lower bound the variance by $ \frac{\phi}{2} \cdot (\frac{1}{2})^2 = \frac{\phi}{8}$. This gives us an overall bound of $O(\frac{m}{\sqrt{n\phi}})$, and therefore $O(\frac{m^3}{\sqrt{n\phi}})$ after a union bound.

    Finally, we show Inequality~\eqref{eq:mode-bound}. Fix a value $\ell$. Let $\tau \in \mathcal{L}(M \setminus \set{a})$ be an arbitrary partial ranking of the candidates without $\ell$. We will write $\sigma \setminus \set{a} = \tau$ when the partial ranking of $\sigma$ without $a$ included matches $\tau$. We will show that when $\sigma$ is sampled from a Mallows model, conditioned on it matching $\tau$, the probability $a$ is $\ell$ positions above $b$ is at most $\frac{1}{1 + \phi}$. Since $\tau$ was arbitrary, by law of total probability, this implies the same bound in general. Indeed, note that once $\tau$ is fixed, there are $m$ possible rankings after the insertion of $a$. At most one can correspond to a difference of $\ell$. Call this ranking $\sigma$. Further, consider inserting $a$ in the neighboring position. We will call this ranking $\sigma'$. Note that the Kendall-tau distance from the starting ranking $\sigma_i$ of $\sigma$ and $\sigma'$ can differ by at most $1$. This implies that $\Pr[\sigma' | \sigma \setminus \set{a} = \tau] / \Pr[\sigma | \sigma \setminus \set{a} = \tau] \ge \phi$. This directly implies that $\Pr[\sigma | \sigma \setminus \set{a} = \tau] \le \frac{1}{1 + \phi}$, as needed.
\end{proof}
This means that $n \in \omega\left(\frac{m^6}{\phi} \right)$ is sufficient. Similar to plurality here, the main requirement on a noise model to satisfy this is that there is no $\ell$ for which two candidates will be $\ell$ steps apart with high probability. As long as this probability is bounded away from $1$, a similar argument should go through.

\textbf{Veto.}
\begin{proposition}[Veto]
    The rate at which \textsc{Veto} smoothed-satisfies \textsc{Resolvability} is at least $1 - n\phi^{m - 2}.$
\end{proposition}
\begin{proof}
    Consider a profile where all voters rank two candidates $a$ and $b$ in their top two positions. We upper bound the probability that either $a$ or $b$ is ranked last by any voter. If this never occurs, then $a$ and $b$ will be tied. To that end, recall that a voter's first choice will be ranked last with probability $\frac{\phi^m}{\sum_{j = 1}^m \phi^j}$, and their second choice will be ranked last with probability $\frac{\phi^{m - 1}}{\sum_{j = 1}^m \phi^j}$. Hence, neither will ranked last with probability at least
    \begin{align*}
        1 - \frac{\phi^{m - 1} + \phi^m}{\sum_{j = 1}^m \phi^j} &= 1 - \frac{\phi^{m -2} + \phi^{m - 1}}{\sum_{j = 0}^1 \phi^j}\\
        &=1 - \frac{(\phi^{m -2} + \phi^{m - 1})(1 - \phi)}{1 - \phi^m}\\
        &= 1 - \frac{(\phi^{m -2} + \phi^{m - 1})(1 - \phi)}{1 - \phi^m}\\
        &= 1 - \frac{\phi^{m -2} -\phi^m}{1 - \phi^m}\\
        &\ge 1 - \phi^{m - 2}.
    \end{align*}
    Hence, union bounding over all voters, we get that no voter will place $a$ or $b$ last with probability at least $1 - n\phi^{m - 2}$. This lower bounds the rate at which veto can smoothed-satisfy resolvability.
\end{proof}
This implies that it is necessary to have $n \in \Omega(\frac{1}{\phi^{m - 2}})$ to ensure \textsc{Veto} smoothed-satisfies \textsc{resolvability}. Note that the main requirement here was that there be an exponentially small probability of a voter moving one of their top two candidates last.

\textbf{Minimax.}
\begin{proposition}[Minimax]
    The rate at which \textsc{Minimax} smoothed-satisfies \textsc{Resolvability} is
    \[\Omega\left( \frac{1}{\sqrt{n\bar{q}(\floor{m/2})}} -  m\exp\left(-\frac{n(1 - 2\bar{q}(\floor{m/2}))^2}{32} \right)\right),\]
    at least for $n$ divisible by $4$.
\end{proposition}
\begin{proof}
    
Fix some $n$ that is divisible by $4$ and first, assume $m$ is even (we will describe how to extend it to the odd case later). Consider the following instance. Let $a$ and $b$ be two candidates and let $C$ and $D$ be a partition of the remaining candidates into two sets of equal size, each having $m/2 - 1$ candidates. Let $\tau^C$ and $\tau^D$ be arbitrary orders of the candidates in $C$ and $D$ respectively, and let $\text{rev}(\tau^C)$ and $\text{rev}(\tau^D)$ be the reversals of these rankings respectively. Finally, assume the voter rankings are as follows, each occurring $n/4$ times: 
\begin{enumerate}
    \item $b \succ \text{rev}(\tau^C) \succ a \succ \tau^D$
    \item $b \succ \text{rev}(\tau^D) \succ a \succ \tau^C$
    \item $a \succ \text{rev}(\tau^C) \succ b \succ \tau^D$
    \item $a \succ \text{rev}(\tau^D) \succ b \succ \tau^C$
\end{enumerate}
We will show that except for with exponentially small probability, $a$ and $b$ still beat every other candidate in a pairwise competition. However, with a reasonably large probability, $a$ and $b$ are pairwise tied. When these events occur, $a$ and $b$ have the same optimal Minimax score of $n/2$, while all others have strictly less, and are hence tied.

For the first, consider an arbitrary candidate $c \in C$. The arguments for if $c \in D$ or with $b$ instead of $a$ will be symmetric. Let $X_i$ be a random variable that is $1$ if $i$ ranks $a$ above $c$ in the final ranking and $-1$ otherwise. We would like to upper bound the probability that $\sum_i X_i \le 0$. We will do this using an application of Hoeffding's inequality. To do this, we must obtain bounds on $\mathbb{E}[\sum_i X_i]$.

Suppose $c$ is ranked $k$'th in $\tau^C$. Note that $c$ is only preferred to $a$ on voters in the first group. For such a voter $i$, as there is a probability $\bar{q}(k)$ of a swap, so $\E[X_i] = 2\bar{q}(k) - 1$. For voters in the second group, $a$ is preferred to $c$ by the same magnitude, hence, for such a voter $i$, $\E[X_i] = 1 - 2\bar{q}(k)$, the exact negative of the first.  For voters in the third group, since $a$ is preferred to $c$, they retain their order with probability at least $1/2$, so for such voters $i$, $\E[X_i] \ge 0$. For voters in the fourth group, $a$ is preferred to $c$ by $|D| + 1 + k$ positions, hence, $\E[X_i] \ge 2 q(|D| + 1 + k) - 1$. Since $\bar{q}$ is decreasing and $|D| + 1 + k \ge m/2$, this is at least $1 - 2\bar{q}(m/2)$. Putting this together, we have that \[\E[\sum_i X_i] \ge n/4*(2q(k)  - 1) + n/4(1 - 2q(k)) + n/4(1 - 2\bar{q}(m/2)) = n/4(1 - 2\bar{q}(m/2)).\]
Plugging this into Hoeffding's inequality, since the variables take on values in $[-1, 1]$, this implies that
\[
    \Pr[\sum_i X_i \le 0] \le \exp\left(-\frac{n(1 - 2\bar{q}(m/2))^2}{32} \right).
\]

Union bounding over all $m$ candidates choices of $c$ and $2$ choices of $a$ and $b$, we get that the probability $a$ and $b$ pairwise beat all other candidates except for with probability $2m\exp\left(-\frac{n(1 - 2\bar{q}(m/2))^2}{32} \right)$.

Next, we consider the relative rankings of $a$ and $b$. Note that on groups one and two, $b$ is beating $a$, and on groups three and four, $a$ is beating $b$. In all cases, the margin of victory is $m / 2$ positions. The probability of a swap on any of these rankings is $\bar{q}(m/2)$. Hence, the number of swaps on the first $n/2$ candidates follows a $\text{Bin}(n/2, \bar{q}(m/2))$ distribution, and symmetrically, so does the number of swaps on the second $n/2$. Candidates $a$ and $b$ will be tied in a pairwise competition if the two (independent) draws from these binomials are equal. We show next that this occurs with probability $\Omega(\frac{1}{\sqrt{n\bar{q}(m/2)}})$ which follows directly from the following lemma.

\begin{lemma}
    The probability two independent draws from a $\text{Bin}(n, p)$ distribution are equal is $\Omega(\frac{1}{\sqrt{np}})$. 
\end{lemma}
\begin{proof}
    Fix an arbitrary $n$ and $p$. Note that the mean of a binomial distribution is $np$. By standard Chernoff bounds, if $X$ follows a $\text{Bin}(n, p)$ distribution, $\Pr[|X - \mu| \ge \delta \mu] \le 2\exp(-\delta^2 \mu / 3)$ for all $\delta \in (0, 1)$ where $\mu=np$ . In particular, plugging in $\delta = 2/\sqrt{\mu}$, we get that with constant probability ($\ge 1 - 2\exp(-4/3) \ge .47$), $X$ is within $2\sqrt{\mu}$ of its mean. Note that there are at most $4\sqrt{np} + 1$ integer values within $2\sqrt{np}$ of the mean. With constant probability ($\ge .47^2$), both binomials will take on one of these values. Conditioned on this event, the probability they are equal is at least $\frac{1}{4\sqrt{np} + 1}$. Indeed, suppose conditioned on being one of these $\frac{1}{4\sqrt{np} + 1}$ values, each was taken with probability $p_1, p_2, \ldots, p_{4\sqrt{np} + 1}$ with $\sum_{i = 1}^{4\sqrt{np} + 1} p_i = 1$. The probability they are equal is $\sum_{i = 1}^{4\sqrt{np} + 1} p^2_i \ge \sum_i \frac{p_i}{4 \sqrt{np} + 1} = \frac{1}{4\sqrt{np} + 1}$. Hence, the probability they are equal is at least $\Omega(\frac{1}{\sqrt{np}})$. 
\end{proof}

Combining the fact that $a$ and $b$ are pairwise tied with probability $\Omega(\frac{1}{\sqrt{n\bar{q}(m/2)}})$ and pairwise beat all others with probability $1 - O\left(\exp(-\frac{n(1 - 2\bar{q}(m/2))^2}{32} \right)$ completes the bound.

To handle $m$ which is odd, we can add a dummy candidate to the end of all the rankings. This candidate wins with even smaller probability, so all of the analysis continues to hold. We simply need to replace $\bar{q}(m/2)$ with $\bar{q}(\floor{m/2})$.
\end{proof}
Note that using the fact that $\bar{q}(\floor{m/2}) \in O(1/\log m)$, a necessary condition for a high probability bound is $n \in \omega(\bar{q}(\floor{m/2})$. We can plug in our various bounds on $\bar{q}(\floor{m/2}$, but for one, this directly implies $n \in \omega(1/(m\phi^{\floor{m/2}}))$ is necessary. In general, the only condition needed on a noise model for an argument like this to work is that it is unlikely for two candidates a distance of $m/2$ apart to swap. 

% \newpage

% Further, assume that within these blocs, alternatives are cycled symmetrically.
% \begin{enumerate}
%     \item $(1-\epsilon)/2$ voters have $a \succ A \succ b \succ B$
%     \item $(1-\epsilon)/2$ voters have $b \succ B \succ a \succ A$
%     \item $\epsilon/2$ voters have $ a \succ B \succ b \succ A$
%     \item $\epsilon/2$ voters have $ b \succ A \succ a \succ B$
% \end{enumerate}
% Notice that both $A$ and $B$'s worst pairwise dominations are magnitude $1-\epsilon$, where $A$ is dominated most by $a$ and $B$ is dominated most by $b$. In contrast, $a$ and $b$'s worst pairwise dominations are magnitude $1/2$, where $a$'s is uniquely most dominated by $b$ and $b$ is uniquely most dominated by $a$.\\



% %\textbf{Claim 0: upper-boun} First, observe that the probability that for something in $B$ (resp. $A$) to become the worst pairwise dominator of $a$ (resp. $b$) requires the sampling of at least one ranking involving at least $3/(m-1)$ swaps. In order for something in $B$ to pairwise dominate $a$ surpass $a$ in the type 1 ranking.


% \noindent \textbf{Claim 1.} \textit{Upper-bounding the probability of anything other than $a$ or $b$ having the smallest pairwise domination.} 

% Since $A$ and $B$ are symmetric, we can just consider a single alternative $x \in A$ without loss of generality. Then, we have to upper-bound the probability of two events:\\

% \textit{Event 1:} \textit{$x$ ends up with a lower pairwise domination than $b$.}\\

% (1.1) First, bounding the probability that $x$ ends up with a lower pairwise domination than $b$. In the original profile, $a$ pairwise dominates $x$ by magnitude $1/2 + \epsilon/2$, owing to the Types 1, 3, and 4. In Type 1, $x$ is always at least $m/2$ positions behind $a$. In Type 3, $x$ is $j$ positions behind
 

% \textit{Event 2:} \textit{$x$ ends up with a lower pairwise domination than $a$}.


% Finally, adding these probabilities (union bound), we conclude the claim.\\

% \noindent \textbf{Claim 2:} \textit{Upper-bounding the probability that $a$'s worst pairwise domination ends up being something other than $b$ (or symmetrically, $b$'s worst pairwise domination being something other than $a$).}\\


% \noindent \textbf{Claim 3:} \textit{Upper-bounding the probability that $a$ and $b$ don't tie. }

% Since $a$ and $b$ are of the same distance apart in every ranking ($(m-2)/3$), by \Cref{lem:no-swap-prob}, they have exactly the same probability of swapping: $q(\frac{m-2}{3})$.
% Now, define the random variable $X_1$ be the probability that $a$ is swapped ahead of $b$ in rankings of type 2 or 4, and let $X_2$ be the probability that $b$ is swapped ahead of $a$ in rankings of type 1 or 3. Since all rankings are perturbed independently, $X_1$ and $X_2$ are both distributed as $Bin(n/2,q(\frac{m-2}{3}))$.

% For Claim 2, this is $\Pr[X_1 = X_2]$ where $X_1, X_2 \sim \text{Bin}(n/2, \phi^m)$ i.i.d.\@. 
% \textcolor{red}{I think $X_1 = X_2$ is not sufficient for a tie; we also need to make sure that $a$'s worst pairwise domination (resp. $b$'s) doesn't become something from $B$ (resp. $A$). I think we have to handle something related in claim 1 --- see red text.}



% \textbf{Conjecture:} $Pr[X_1 \in [n/2*q \pm \sqrt{n q/2} ] \geq C.$
% (probably use Chernhoff)

% This implies that the two binomials have to equal with probability at least $\frac{C}{2\sqrt{nq/2}}$.

% $\Pr[|X - \mu| \ge \delta \mu] \le \exp(-\delta^2 \mu /3)$ so setting $\delta = 1/\sqrt{\mu}$ gets constant ($1 - 1/e^{1/3}$). So with constant probability you are within $\sqrt{\mu} = \sqrt{nq/2}$ for us.

% For veto, ranking will be
% \begin{enumerate}
%     \item $1/2: a \succ b \succ C$
%     \item $1/2: b \succ a \succ C$
% \end{enumerate}
% and make sure everybody else appears last at least $1/m$ of the time. Hopefully: probability first place is last $\propto \phi^{m- 1}$ and second place last $\propto$



% \paragraph{Kemeny Young.}
% \begin{itemize}
%     \item $1/2 - 1/n$ with $a \succ \tau_C \succ b\succ \tau_D $
%     \item $1/2 - 1/n$ with $b \succ rev(\tau_D) \succ a \succ rev(\tau_C)$
%     \item $1$ with $\tau_C \succ a \succ b \succ \tau_D$
%     \item $1$ with $\tau_D \succ b \succ a \succ \tau_C$
% \end{itemize}




% \begin{proposition}[Veto]
%     The rate at which
% \end{proposition}
% \begin{proof}
%     Consider the following instance. We will have two candidates $a$ and $b$. $n/2$ voters will have ranking $a \succ b \succ \cdots$ and the remaining will have ranking $b \succ a \succ \cdots$. The bottom part of their ranking will be arbitrary, just done in such a way that all other candidates appear for at least $n/m$ voters. We will that except for with exponentially small probability.
% \end{proof}

% Alternative veto:

==> 5discussion.tex <==
\section{Extensions and Discussion}\label{sec:discussion}




\subsection{Extensions to Arrow's Theorem (and other multi-axiom impossibilities)} \label{sec:extensions}

\noindent \textbf{Other multi-axiom impossibilities.} 

